Increasing Domain Infill Asymptotics for Stochastic Differential Equations Driven by Fractional Brownian Motion

Although statistical inference in stochastic differential equations (SDEs) driven by Wiener process has received significant attention in the literature, inference in those driven by fractional Brownian motion seem to have seen much less development in comparison, despite their importance in modeling long range dependence. In this article, we consider both classical and Bayesian inference in such fractional Brownian motion based SDEs. In particular, we consider asymptotic inference for two parameters in this regard; a multiplicative parameter associated with the drift function, and the so-called "Hurst parameter" of the fractional Brownian motion, when the time domain tends to infinity. For unknown Hurst parameter, the likelihood does not lend itself amenable to the popular Girsanov form, rendering usual asymptotic development difficult. As such, we develop increasing domain infill asymptotic theory, by discretizing the SDE. In this setup, we establish consistency and asymptotic normality of the maximum likelihood estimators, as well as consistency and asymptotic normality of the Bayesian posterior distributions. However, classical or Bayesian asymptotic normality with respect to the Hurst parameter could not be established. We supplement our theoretical investigations with simulation studies in a non-asymptotic setup, prescribing suitable methodologies for classical and Bayesian analyses of SDEs driven by fractional Brownian motion. Applications to a real, close price data, along with comparison with standard SDE driven by Wiener process, is also considered. As expected, it turned out that our Bayesian fractional SDE triumphed over the other model and methods, in both simulated and real data applications.

==> realdata.tex <==
\section{Application to real data}
\label{realdata}
To deal with real data we collect the close price of a particular company from stock market data 
($460$ observations during the time range August $5$, 2013, to June $30$, 2015)  which is available on {\it www.nseindia.com}. 

A simple autocorrelation plot of the close price data revealed autocorrelations close to one, even for lag greater than $25$, suggesting long-range dependence. 
Thus, an $SDE$ driven by a fractional Brownian motion seems to be appropriate here. 
Moreover, for simplicity we fix the choice of the ratio $B(t,X_t)/C(t,X_t)$ as a constant; in fact, we set $B(t,X_t)=C(t,X_t)=X^{\nu}_t$, where $\nu>0$ is to be
determined appropriately, following the discussion below. 

In other words, we propose the following form of such $SDE$:
\begin{equation*}
	dX_t=\beta X_t^{\nu}dt + \gamma X_t^{\nu}dW_t^H,
	%\label{eq:sde_real}
\end{equation*}
where $\nu>0$ is to be chosen such that both classical and Bayesian analyses of the data using the above $SDE$ supports values of $H$ close to one. As it turned out,
$\nu=3/2$ is an appropriate choice in this regard. In other words, we fit the following $SDE$ to the close price data with respect to both classical and Bayesian setups:
\begin{equation}
dX_t=\beta X_t^{3/2}dt + \gamma X_t^{3/2}dW_t^ H
	\label{eq:sde_real}
\end{equation}
Here $\beta$, $H$ and $\gamma$ are unknown parameters which need to be learned about. However, as is the case in most statistical applications of $SDE$,
we choose to assume $\gamma$ as given. In both classical and Bayesian setups 
we choose $\gamma$ to minimize the average lengths of the 95\% confidence and credible intervals, respectively, associated with the held-out observations, subject
to inclusion of all the held-out data points.
In our application we consider the first $400$ data points as given and predict the next $60$ data points in both classical and Bayesian setups. 
The values of $\gamma$ thus obtained would be considered as given for prediction of actual future observations. 


\subsection{Real data analysis in the classical setup}
\label{subsec:classical_real}
Starting from arbitrary initial values of $\btheta = (\beta,H)$ we performed simulated annealing aided with a TMCMC algorithm 
that has provision for further enhancement of mixing properties to obtain the $MLE$ of $\btheta$. Our algorithm is provided below as Algorithm \ref{algo:sima_real}. 
\begin{algorithm}
\caption{Simulated annealing aided by TMCMC with enhanced mixing properties}
\label{algo:sima_real}
\begin{itemize}
	\item[(1)] Begin with an initial value $\btheta^0=\left(\beta^{(0)},H^{(0)}\right)$.
%\item[(2)] For enhancement of mixing properties, set $p_1=q_1=1/2$.
\item[(2)] For $t=1,\ldots,N$, do the following:
	\begin{enumerate}
		\item[(i)] Generate $\varepsilon_1\sim N(0,1)$, $\varepsilon_2\sim U(-1,1)$, $b_j\stackrel{iid}{\sim}U(\{-1,1\})$ for $j=1,2$, $U_1\sim U(0,1)$. If $U_1<1/2$, create $\tilde\beta=\beta^{(t-1)}+b_1a_1|\varepsilon_1|$ and $\tilde H=H^{(t-1)}+b_2a_2|\varepsilon_1|$. Else, set $\tilde\beta=\beta^{(t-1)}{\varepsilon_2}^{b_1}$ and $\tilde H=H^{(t-1)}{\varepsilon_2}^{b_2}$.  
			Let $\tilde\btheta=\left(\tilde\beta,\tilde H\right)$.
		\item[(ii)] Evaluate 
			$$\alpha_1=\min\left\{1,\exp\left\{\frac{\ell_{T,n}\left(\tilde\btheta\right)-\ell_{T,n}\left(\btheta^{(t-1)}\right)+\log (J)}{\tau_t}\right\}
			I_{(0,1)}(\tilde H)\right\},$$
			where $\tau_t=\frac{1}{\log(t)}$ when $t\geq 100$ and $t^{-1}$ otherwise and $J$ is the Jacobian of corresponding transformation. ($J = 1$ in additive case and $J={|\varepsilon_2|}^{\sum b_j}$ in multiplicative case)
		\item[(iii)] Set $\btheta^{(t)}=\tilde\btheta$ with probability $\alpha_1$, else set $\btheta^{(t)}=\btheta^{(t-1)}$.

   To provide further mixing,
                  \item[(iv)] Generate $\varepsilon_3\sim N(0,1)$,  $U_2\sim U(0,1)$. If $U_2<1/2$  ,

    Further generate $u_1\sim U(0,1)$. If $u_1<1/2$, create $\beta^*=\beta^{(t)}+a_1|\varepsilon_3|$ and $H^*=H^{(t)}+a_2|\varepsilon_3|$. 
			Else, set $\beta^*=\beta^{(t)}-a_1|\varepsilon_3|$ and $H^*=H^{(t)}-a_2|\varepsilon_3|$. 

If $U_2\geq 1/2$,
  
Generate $\varepsilon_4\sim U(-1,1)$, $u_2\sim U(0,1)$. If $u_2<1/2$, create $\beta^*=\beta^{(t)}\varepsilon_4$ and $H^*=H^{(t)}\varepsilon_4$. Else, set $\beta^*=\beta^{(t)}/\varepsilon_4$ and $H^*=H^{(t)}/\varepsilon_4$.
Let $\btheta^*=\left(\beta^*,H^*\right)$.
		\item[(v)] Evaluate 
			$$\alpha_2=\min\left\{1,\exp\left\{\frac{\ell_{T,n}\left(\tilde\btheta\right)-\ell_{T,n}\left(\btheta^{(t-1)}\right)+\log (J)}{\tau_t}\right\}
			I_{(0,1)}(\tilde H)\right\},$$
			where $\tau_t=\frac{1}{\log(t)}$ when $t\geq 100$ and $t^{-1}$ otherwise and $J$ is the Jacobian of corresponding transformation. (In the case of $U_2<1/2$, $J = 1$  and otherwise, $J={|\varepsilon_2|}^2$ or $J={|\varepsilon_2|}^{-2}$  correspondingly)
		\item[(vi)] Accept $\btheta^*$ with probability $\alpha_2$ or remain at $\btheta^{(t)}$. To avoid notational complexity whether it is $\btheta^*$ or $\btheta^{(t)}$ we write final value of each iteration as $\btheta^{(t)}$.
	\end{enumerate}
\item[(3)] From the sample $\left\{\btheta^{(j)};j=0,1,\ldots,N\right\}$, set $\hat\btheta_{T,n}=\btheta^{(j^*)}$ where 
	$\btheta^{(j^*)}=\underset{j=0,1,\ldots,N}{\arg\max}~\ell_{T,n}\left(\btheta^{(j)}\right)$.
\end{itemize}
\end{algorithm}

In our application, initial values are arbitrarily chosen and we set $N=10^4$ and $a_1=a_2=0.0005$. With the obtained $MLE$ given a specific value of $\gamma$ we 
predicted the close price of next $60$ days for that company in two ways. In the first way, at every step each data point is predicted with the 
consideration that data values at the previous time point is given beforehand, that is, one-step-ahead forecast is obtained. 
In the other way, starting from the 400th data point, predictions for the next 60 data points are obtained, which is the $60$-step-ahead forecast. 
To obtain desired confidence intervals for the forecasts, we generated $10,000$ realizations of size $60$ from the $SDE$ (\ref{eq:sde_real}) given the first $400$
data points.
%after replacing $\btheta$ in (\ref{eq:sde_real}) with the $MLE$ $\hat\btheta$ and the specific value of $\gamma$, and these $10,000$ datasets yielded the distributions
%associated with the held-out data points, using which we computed their $95\%$ and $50\%$ confidence intervals. 
We repeated the calculations for different values of $\gamma$, from which we obtained the 
final value of $\gamma$ as the one which yielded minimum average length of the 95\% confidence interval.
Associated with the final vaue of $\gamma$, we also report the number of held-out data points that fail to lie within the 95\% and the 50\% confidence intervals.

%In each case 95\% and 50\% confidence intervals are 
%calulated and no. of data lying outside the confidence intervals are detected in both the cases. The average length of 95\% confidence interval is also noted for comparison with the Bayesian set up. 

We repeated the entire procedure of classical analysis for the case where the $SDE$ is assumed to be driven by Brownian motion instead of fractional Brownian motion. 
In the latter case, as $H=0.5$ corresponds to Brownian motion, the only unknown parameter is $\beta$ and $\gamma$ is fixed in the same way as in the fractional set up. 
This analysis facilitates comparison of fractional $SDE$ model with the more usual $SDE$ models driven by Brownian motion.

For the classical analysis $\gamma$ is found to be $165$ and $0.4$ for our $SDE$s driven by fractional and standard Brownian motion, respectively. 
The results are tabulated in Tables \ref{table:classical_real_fBm} and \ref{table:classical_real_Bm} showing the $MLE$s of $H$ and $\beta$, the values
of $\gamma$ for one step ahead and $60$ steps ahead forecasts, the number of held-out data points outside the correspondng 50\% and 95\% confidence intervals $(CI$)
and the average length of the 95\% CIs of the held-out data points.
Observe that compared to fractional $SDE$, the average lengths of the 95\% CI are small for standard $SDE$, but a significantly larger number of held-out observations
are excluded from the 50\% $CI$s of the standard $SDE$. This indicates that compared to standard $SDE$, most of the held-out observations are concentrated
in the high-density regions of the fractional $SDE$. 
Hence, the fractional $SDE$ clearly outperforms the standard $SDE$.

The densities associated with fractional and standard $SDE$s are displayed in Figures 
\ref{fig:1_60_classical_fBM} and \ref{fig:1_60_classical_BM}, respectively, where higher densities are represented by progressively intense colours;
the thick, black line stands for the held-out observed data. These figures are the detailed versions of Tables 
\ref{table:classical_real_fBm} and \ref{table:classical_real_Bm}.

\begin{table}[h]
\centering
\caption{Results of classical analysis of real data modeled by fractional $SDE$.}
\label{table:classical_real_fBm}
	\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$\hat H_{T,n}$ & $\hat \beta_{T,n}$ & $\gamma$ & step & \# outside 50\% $CI$ & \# outside 95\% $CI$ & Average length of 95\% $CI$\\ 
\hline
	0.995  &  -0.002578  &  165  &  1  &  24  & 1 & 31.11014\\
	0.995  &  -0.002578  &  165 &  60  &  17  &  0 & 155.5142\\
%	0.995  &  -0.001224  &  158  &  1  &  25  &  1 & 31.08635\\
%	0.995  &  -0.001224  &  158  &  60  & 17  &  0 & 157.1585\\   
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Results of classical analysis of real data modeled by standard $SDE$.}
\label{table:classical_real_Bm}
	\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
%$H$ & $\hat \beta_{T,n}$ & $\gamma$ & step & no. of data outside 50\% $CI$ & no. of data outside 95\% $CI$ & average 95\% $CI$\\ 
$H$ & $\hat \beta_{T,n}$ & $\gamma$ & step & \# outside 50\% $CI$ & \# outside 95\% $CI$ & Average length of 95\% $CI$\\ 
\hline
	0.5  &  0.00021  &  0.4  &  1  &  38  & 2 & 25.20115\\
	0.5  &  0.00021  &  0.4 &  60  &  24  &  0 & 122.7201\\
%	0.5  &  0.00021  &  1  &  1  &  5  &  0 & 62.96177\\
%	0.5  &  0.00021  &  1  &  60  & 0 &  0 & 333.4945\\   
\hline
\end{tabular}
\end{table}

\begin{figure}
\centering
\subfigure []{ \label{fig:c1_165}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI1_165.pdf}}
\hspace{2mm}
%\subfigure []{ \label{fig:c1_158}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI1_158.pdf}}\\
%\vspace{2mm}
\subfigure []{ \label{fig:c60_165}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI60_165.pdf}}
%\hspace{2mm}
%\subfigure []{ \label{fig:c60_158}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI60_158.pdf}}\\
\caption{One step ahead and 60 steps ahead forecasts in the classical setup corresponding to fractional $SDE$.}
\label{fig:1_60_classical_fBM}
\end{figure}


\begin{figure}
\centering
%\subfigure []{ \label{fig:c1_bm1}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI1_bm_1.pdf}}
%\hspace{2mm}
\subfigure []{ \label{fig:c1_bm0.4}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI1_bm_0.4.pdf}}
%\vspace{2mm}
%\subfigure []{ \label{fig:c60_bm1}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI60_bm_1.pdf}}
\hspace{2mm}
\subfigure []{ \label{fig:c60_bm0.4}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI60_bm_0.4.pdf}}\\
\caption{One step ahead and 60 steps ahead forecasts in the classical setup corresponding to standard $SDE$.}
\label{fig:1_60_classical_BM}
\end{figure}



%In Bayesian set up, $\gamma=158$ and $\gamma=1$ corresponding to the fractional $SDE$ and standarad $SDE$. 
%For better understanding of the choice of model, both classical and Bayseian investigations are carried out for $\gamma=165$ and $\gamma=158$ in fractional $SDE$ 
%framework and $\gamma=0.4$ and $\gamma=1$ in standard $SDE$ setup.
%
%Our figures represent 95\% cofidence intervals in all cases where real data is shown by black line and all the results are tabulted in the 
%Table \ref{table:classical_real_fBm}, Table \ref{table:classical_real_Bm}, Table \ref{table:bayesian_real_fBm} and Table \ref{table:bayesian_real_Bm}. 
%In classical setup, $MLE$ is denoted by $\hat H_{T,n}$ and $\hat \beta_{T,n}$ whereas in Bayesian case median of posterior realizations is mentioned 
%in each case and denoted by $H^*$ and $\beta^*$.

\subsection{Real data analysis in the Bayesian setup}
\label{subsec:bayesian_real}

In the Bayesian setup, we first reparameterize $H$ as $H=\exp(\nu)/(1+\exp(\nu))$ as in
Section \ref{subsec:bayesian_simstudy} and assume {\it a priori} that $\nu\sim N\left(\nu_{T,n},\sigma^2_{\nu}\right)$ and 
$\beta\sim N\left(\mu_{\beta},\sigma^2_{\beta}\right)$, where $\mu_{\beta}=0.001, \sigma_{\nu}=\sigma_{\beta}=0.1$. 
As in Section \ref{subsec:bayesian_simstudy}, $\nu_{T,n}$ is set as $\log\left(\frac{\hat H_{T,n}}{1-\hat H_{T,n}}\right)$.

For Bayesian inference, a TMCMC algorithm with enhanced mixing properties is considered similar to Algorithm \ref{algo:sima_real}
where $\nu$ is updated instead of $H$ and the acceptance probability becomes 
$\alpha=\min\left\{1,\exp\left\{\ell_{T,n}\left(\tilde\btheta\right)-\ell_{T,n}\left(\btheta^{(t-1)}\right)+\log (J)\right\}\right\}$. 
In our application, we set $N=10^4$ and $a_1=a_2=0.05$. 

Posterior predictive distributions of the $60$ held-out observations are obtained in two ways similar to that of the classical set up.
%by the realizations $\left\{\btheta^{(t)};t=0,1,\ldots,N\right\}$. 
In each case, whether it is one step ahead or 60 steps ahead predictions, 95\% and 50\% Bayesian credible intervals are obtained and the number of data points lying outside 
correspoding regions are also noted. Again, $\gamma$ is treated as a fixed parameter whose value is obtained by minimizing the average length of the
95\% credible intervals subject to their inclusion of all the respective held-out observations. Once again we remind the reader that this fixed value of $\gamma$ would
be used even for actual forecasting future observations.
%within their respective 95\% credible intervals. Average length of 95\% credible region for each data is also obtained. 

The whole analysis is carried out for the standard $SDE$ driven by Wiener process, that is, with $H=0.5$ 
and in this case we are interested in the posterior of $\beta$ only as $\gamma$ is fixed in the way as explained above.

In this Bayesian set up, we obtain $\gamma=158$ and $\gamma=1$ for fractional and standard $SDE$, respectively, corresponding to
which Tables \ref{table:bayesian_real_fBm} and \ref{table:bayesian_real_Bm} provide the results of our Bayesian analyses.
In the tables $H^*$ and $\beta^*$ stand for the respective posterior medians and Bayesian credible interval is denoted by $BCI$.
Note that the average length of 95\% $BCI$ for standard $SDE$ is much larger compared to that for fractional $SDE$ and hence it is no surprise
that even those for 50\% $BCI$s would be much larger for the former and hence excludes less number of observations. Indeed, the average lengths for
standard $SDE$ are much larger even compared to both the classical analyses reported in Tables \ref{table:classical_real_fBm} and \ref{table:classical_real_Bm},
and thus it is clear that the standard $SDE$ fails to outperform the fractional $SDE$. It is also clear, in terms of adequate average lengths of the 
95\% $BCI$ and the number of held-out observations falling in the high-density regions, that our Bayesian fractional $SDE$ is the best performer.

The posterior predictive densities associated with fractional and standard $SDE$s are displayed in Figures 
\ref{fig:1_60_Bayesian_fBM} and \ref{fig:1_60_Bayesian_BM}, respectively, where higher posterior predictive densities are represented by progressively intense colours;
the thick, black line stands for the held-out observed data, as before.
%For better understanding of the choice of model, both classical and Bayseian investigations are carried out for $\gamma=165$ and $\gamma=158$ 
%in fractional $SDE$ framework and $\gamma=0.4$ and $\gamma=1$ in standard $SDE$ setup.
\begin{table}[h]
\centering
\caption{Results of Bayesian analysis of real data modeled by fractional $SDE$.}
\label{table:bayesian_real_fBm}
	\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$ H^*$ & $\beta^*$ & $\gamma$ & step & \# outside 50\% $BCI$ & \# outside 95\% $BCI$ & Average length of 95\% $BCI$\\ 
\hline
%	0.991  &  0.00085  &  165  &  1  &  23  & 1 & 32.87207\\
%	0.991  &  0.00085  &  165 &  60  &  7  &  0 & 210.0178\\
	0.991  &  0.00121  &  158  &  1  &  25  &  1 & 31.472\\
	0.991  &  0.00121  &  158  &  60  & 8  &  0 & 201.4972\\   
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Results of Bayesian analysis of real data modeled by standard $SDE$.}
\label{table:bayesian_real_Bm}
	\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$H$ & $\beta^*$ & $\gamma$ & step & \# outside 50\% $BCI$ & \# outside 95\% $BCI$ & Average length of 95\% $BCI$\\ 
\hline
%	0.5  &  0.00032  &  0.4  &  1  &  38  & 2 & 25.1918\\
%	0.5  &  0.00032 &  0.4 &  60  &  24  &  0 & 125.3408\\
	0.5  &  0.00035  &  1  &  1  &  6  &  0 & 62.98049\\
	0.5  &  0.00035 &  1  &  60  & 0 &  0 & 334.7808\\   
\hline
\end{tabular}
\end{table}


\begin{figure}
\centering
%\subfigure []{ \label{fig:c60_165}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI60_165.pdf}}
%\hspace{2mm}
%\subfigure []{ \label{fig:c60_158}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI60_158.pdf}}\\
%\vspace{2mm}
%\subfigure []{ \label{fig:p60_165}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/PP60_165.pdf}}
%
\subfigure []{ \label{fig:p1_158}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/PP1_158.pdf}}
\hspace{2mm}
\subfigure []{ \label{fig:p60_158}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/PP60_158.pdf}}\\
\caption{One and 60 steps ahead forecasts in the Bayesian setup corresponding to fractional $SDE$.}
\label{fig:1_60_Bayesian_fBM}
\end{figure}

\begin{figure}
\centering
%\subfigure []{ \label{fig:c1_bm1}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI1_bm_1.pdf}}
%\hspace{2mm}
%\subfigure []{ \label{fig:c1_bm0.4}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/CI1_bm_0.4.pdf}}\\
%\vspace{2mm}
\subfigure []{ \label{fig:p1_bm1}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/PP1_bm_1.pdf}}
\hspace{2mm}
\subfigure []{ \label{fig:p60_bm1}
\includegraphics[width=6.5cm,height=5.5cm]{Plot2/PP60_bm_1.pdf}}
%\subfigure []{ \label{fig:p1_bm0.4}
%\includegraphics[width=6.5cm,height=5.5cm]{Plot2/PP1_bm_0.4.pdf}}\\
\caption{One and 60 steps ahead forecasts in the Bayesian setup corresponding to standard $SDE$.}
\label{fig:1_60_Bayesian_BM}
\end{figure}


